Deterministic Algorithmic Approaches to Solve Generalised Wordle

Wordle is a single-player word-based game where the objective is to guess the 5-letter word in a maximum of 6 tries. The game was released to the public in October 2021 and has since gained popularity with people competing against each other to maintain daily streaks and guess the word in a minimum number of tries. There have been works using probabilistic and reinforcement learning based approaches to solve the game. Our work aims to formulate and analyze deterministic algorithms that can solve the game and minimize the number of turns required to guess the word and do so for any generalized setting of the game. As a simplifying assumption, for our analysis of all the algorithms we present, we assume that all letters will be unique in any word which is part of our vocabulary. We propose two algorithms to play Wordle - one a greedy based approach, and other based on Cliques. The Greedy approach is applicable for both hard and easy modes of Wordle, while the Clique formation based approach only works on the Easy mode. We present our analysis on both approaches one by one, next.

==> clique_algos/archived/Algorithm_0_AL.tex <==
\subsubsection{Graph Formation}
\begin{algorithm}
\caption{Form Graph Helper}\label{alg:form-graph-helper}
\begin{algorithmic}[1]
\Require $wordle\_tracker$: the Wordle tracker object, $hard$: boolean indicating whether to use hard or soft constraints
\Ensure $graph$: adjacency list representation of the graph, $edge\_exists$: boolean indicating whether an edge exists in the graph
\Function{FormGraphHelper}{$wordle\_tracker, hard$}
  \State $edge\_exists \gets \textbf{False}$
  \State $vocab \gets wordle\_tracker.vocab$
  \State $graph \gets [[] \text{ for } i \text{ in } \text{range}(\text{len}(vocab))]$
  \State $allowed\_unseen\_common \gets 0$
  \If{not $hard$}
    \State $allowed\_unseen\_common \gets 1$
  \EndIf
  \For{$i \textbf{ in } \text{tqdm}(\text{range}(\text{len}(vocab)))$}
    \State $w1 \gets vocab[i]$
    \If{$w1 \text{ in } wordle\_tracker.discarded\_words$}
      \State $\textbf{continue}$
    \EndIf
    \For{$j \textbf{ in } \text{range}(i+1, \text{len}(vocab))$}
      \State $w2 \gets vocab[j]$
      \State $words\_intersection \gets \text{set}(vocab[i]) \cap \text{set}(vocab[j])$
      \State $common\_unseen\_letters \gets words\_intersection \cap wordle\_tracker.unseen\_chars$
      \If{$\text{len}(common\_unseen\_letters) == allowed\_unseen\_common$}
        \State $graph[i].\textbf{append}(j)$
        \State $graph[j].\textbf{append}(i)$
        \State $edge\_exists \gets \textbf{True}$
      \EndIf
    \EndFor
  \EndFor
  \State \textbf{return} $graph$, $edge\_exists$
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Form Graph}\label{alg:form-graph}
\begin{algorithmic}[1]
\Require $wordle\_tracker$: the Wordle tracker object
\Ensure $graph$: adjacency list representation of the graph, $edge\_exists$: boolean indicating whether an edge exists in the graph
\Function{FormGraph}{$wordle\_tracker$}
  \State $new\_graph, edge\_exists \gets \text{FormGraphHelper}(wordle\_tracker, hard=True)$
  \If{not $edge\_exists$}
    \State $new\_graph, edge\_exists \gets \text{FormGraphHelper}(wordle\_tracker, hard=False)$
  \EndIf
  \State \textbf{return} $new\_graph$, $edge\_exists$
\EndFunction
\end{algorithmic}
\end{algorithm}

"FormGraph" takes a WordleTracker object and calls the "FormGraphHelper" function with the hard parameter set to True. If there are no edges in the graph returned by "FormGraphHelper", the function calls "FormGraphHelper" function with the hard parameter set to "False" . We make this hard and soft graph creation different to allow for more chances of edge creation in case of there being no two words having all distinct letters between them in some specific vocabulary. The soft graph creation allows for some lax and permits 1 letter to be common. Note that this has nothing to do with hard and soft game modes of the wordle game itself.

The "FormGraphHelper"  function takes a WordleTracker object and a boolean hard, which is True by default to allow for no common letters. The function creates an empty graph with an adjacency list data structure. It then sets the number of allowed common unseen letters between two words based on the value of hard to be generalizable for if and when it is called for soft graph creation case. For each word in the vocabulary, it checks if the word has already been discarded by the WordleTracker object. If so, it skips the word and moves on to the next word. Otherwise, it compares the current word with every other word in the vocabulary that comes after it. If the two words have the required number of common unseen letters(0 for hard and 1 for soft), an edge is added between the two vertices in the graph. The edge is bidirectional, so it is added to the adjacency list of both vertices. The EdgeExists flag is set to True if any edges were added to the graph. Finally, the function returns the graph and the EdgeExists flag.

\textbf{Time Complexity}:The time complexity of the graph creation algorithm depends on the number of words in the input wordleTracker object, denoted by n. The time complexity of the algorithm is $O(n^2)$, as it needs to compare every pair of words. If the graph does not have any edge added to it due to non zero number of common letters(hard graph creation case), then the graph will be created through soft case where 1 unseen characters is allowed to be common, and the added time complexity will be $O(n^2)$. So, worst case the algorithm to create graph will run for $O(n^2)+O(n^2)$ which is $O(n^2)$


\textbf{Claim}: The Graph formed is correct, ie, any two words that do not share any common letters (hard) have a vertex between them and no extra edges exist, ie, edges between pair of words that have any common letter(hard) (or at max 1 common letter in soft)

\textbf{Proof}: This is because we go over each pair of words and add vertics based on these conditions. Further, no extra edges, ie, edges between words that share any letters are added to the graph as well since they do not satisfy the condition for addition of edges. In case of soft mode, only 1 common letter is allowed as highlighted by change in condition.


\subsubsection{Finding K cliques}

\begin{algorithm}[H]
\label{alg:find_clique}
\caption{Finding K-Cliques in a Graph}
\begin{algorithmic}[1]
\Require{An adjacency list, ${adjList}$, and an integer, $k$.}
\Ensure{A list of all $k$-cliques in $adjList$.}
\Function{findKclique}{$adjList, k$}
\State $cliques \gets []$
\Procedure{backtrack}{$current_clique, neighbours$}
\If{length of $currentClique$ is equal to $k$}
\State append $currentClique$ to $cliques$

\Else
\State $lastVertex \gets$ last element of $currentClique$
\For{vertex in $neighbours$}
\State $newNeighbours \gets neighbours \cap$ set of vertices adjacent to $vertex$
\If{vertex $>$ $lastVertex$}
\State $nextClique \gets currentClique$ with $vertex$ appended
\State backtrack($nextClique$, $newNeighbours$)
\EndIf
\EndFor
\EndIf
\EndProcedure
\For{index, vertex in enumerate($adjList$)}
\State backtrack($[index]$, set of vertices adjacent to $vertex$)
\EndFor
\State \Return{$cliques$}
\EndFunction
\end{algorithmic}
\end{algorithm}

The algorithm "Finding K-Cliques in a Graph"  takes in an adjacency list and an integer k, and returns a list of all k-cliques in the given graph represented by the adjacency list. The function makes use of a recursive backtracking algorithm to find all the cliques of size k. The algorithm works by iterating over each vertex in the graph and starting a backtrack from that vertex with a clique of size 1. The backtracking function takes in the current clique and a set of neighbouring vertices, and checks whether the current clique is of size k. If it is, the current clique is added to the list of cliques. Otherwise, the backtracking function loops over each neighbouring vertex and creates a new clique by appending that vertex to the current clique if the vertex is greater than the last vertex in the current clique. The reason for checking if vertex is greater than lastVertex in the backtrack function is to avoid generating duplicate cliques. This is because, starting from some vertex $v_i$ and then choosing some vertex $v_j$ is the same as starting from $v_j$ and then choosing $v_i$. Therefore, we can impose an arbitrary ordering on the vertices and only consider vertices that come after the last vertex in the current clique. 
The new clique is then passed recursively to the backtracking function along with the set of neighbours of the new vertex. The function then returns the list of all k-cliques that were found in the graph.

\textbf{Time Complexity :}The time complexity of this "Finding K-Cliques in a Graph" is exponential, specifically $O(n^k)$ where n is the number of vertices in the graph and k is the size of the cliques being searched for.

\textbf{Claim} : The K clique for the given input graph is found correctly.
\\
\textbf{Proof :}We can use induction on the size of the cliques being searched for (k). 

Base Case: For k=2, the function is simply finding all edges in the graph, which is trivial.

Induction Hypothesis: Now, Assume that the function works correctly for all values of k less than or equal to some integer m. 

To Prove: We want to prove that the function works correctly for k=m+1. First, note that if the graph has no cliques of size m+1 or greater, then the function returns an empty list, which is correct. Now consider a graph that has a clique of size m+1. For each vertex in the graph, the function finds all cliques of size m+1 that contain that vertex. This is done by recursively exploring all the vertices that are adjacent to the current vertex and have not already been included in the clique.

By the induction hypothesis, the function works correctly for cliques of size m, so we can assume that when the function is called recursively with a smaller clique size, it correctly finds all cliques of that size containing the given vertex.
 Therefore, when the function is called recursively with a clique size of m+1, it correctly finds all cliques of that size containing the given vertex. Since this is done for every vertex in the graph, the function correctly finds all cliques of size m+1 in the graph.



\subsubsection{Checking All Anagrams}

\begin{algorithm}[H]
\caption{checkAllAnagrams}
\label{check_all_anagrams}
\begin{algorithmic}[1]
\Require A Wordle tracker object $WordleTracker$ and the hidden word $HiddenWord$
\Ensure The updated Wordle tracker object $WordleTracker$ after checking all anagrams
\State Initialize an empty dictionary $HiddenWordFict$
\State Initialize an empty dictionary $currGuessDict$
\For{each character $ch$ in $hiddenWord$}
\State Add $ch$ as a key to $hiddenWordFict$ with value as its index
\EndFor
\For{each key $ke$ and value $va$ in $WordleTracker.letterPositions$}
\State Add $ke$ as a key to $CurrGuessDict$ with value as $va$
\EndFor
\While{the length of $wordleTracker.letterPositions$ is less than the length of $hiddenWord$}
\State Get all yellow letters by subtracting the letters found from the letter positions
\State Get all yellow positions by subtracting the letter positions from the range of length of hidden word
\State Initialize $shift$ as 0
\State Set $infoFound$ to False
\While{$infoFound$ is False}
\State Initialize a temporary list $allYellowPositionsTmp$ with the shifted positions of $allYellowPositions$
\State Update the current guess dictionary with the shifted positions
\State Initialize an empty list $guessedWordString$
\For{each key $ch$ and value $pos$ in $currGuessDict$}
\State Set the character at $pos$ in $guessedWordString$ as $ch$
\EndFor
\State Convert $guessedWordString$ to a string
\If{$guessedWordString$ is not in $wordleTracker.wordsGuessed$}
\State Add $guessedWordString$ to $wordleTracker.wordsGuessed$
\EndIf
\For{each true character $trueCh$ and true position $truePos$ in $hiddenWordDict$}
\If{$currGuessDict[trueCh] = truePos$ and $trueCh$ is in $allYellowLetters$}
\State Set $infoFound$ to True
\State Add the true character and its true position to the letter positions dictionary
\EndIf
\EndFor
\State Increment $shift$ by 1
\EndWhile
\EndWhile
\State Initialize an empty list $guessedWordString$
\For{each key $ch$ and value $pos$ in $wordleTracker.letterPositions$}
\State Set the character at $pos$ in $guessedWordString$ as $ch$
\EndFor
\State Convert $guessedWordString$ to a string
\If{$guessedWordString$ is not in $wordleTracker.wordsGuessed$}
\State Add $guessedWordString$ to $wordleTracker.wordsGuessed$
\EndIf
\State \Return $wordleTracker$
\end{algorithmic}
\end{algorithm}


The checkAllAnagrams function takes in a wordleTracker object and a hiddenWord string as input. The purpose of the function is to check all possible anagrams of the letters in hiddenWord and determine which one is the true guess word. The function first creates two dictionaries: hiddenWordDict and currGuessDict. hiddenWordDict maps each letter in hiddenWord to its corresponding index in the word, while currGuessDict maps each letter in the wordleTracker object's letterPositions dictionary to its corresponding position in the current guess word. The function continues until all letters in hiddenWord have been found by creating two lists: allYellowLetters and allYellowPositions. AllYellowLetters contains all the letters that have been found but their positions are not yet known, while allYellowPositions contains all the positions that have not yet been filled with a letter. This has a shifting logic to try out all yellow letters in different positions until some new information is found from them. This shifting logic is also explained at the end.\\
The function then enters another loop that shifts the positions of the letters in allYellowLetters and assigns them to the positions in allYellowPositions. It updates currGuessDict with the new positions of the letters in allYellowLetters. The shifting logic ensures that the function considers all possible combinations of the unknown letters in hiddenWord until the correct guess is found. The function  creates a guessedWordString by filling in the known letters in their correct positions and leaving the unknown letters as underscores. If the guessedWordString has not already been guessed, it is added to the wordleTracker object's wordsGuessed list. It then checks if any of the unknown letters in hiddenWord can be deduced from the current guessedWordString. If so, the letter is added to the wordleTracker object's letterPositions dictionary with its correct position. The loop continues until all letters in hiddenWord have been found. Finally, the function creates a guessedWordString with all the letters in their correct positions and returns the updated wordleTracker object.

\emph{Shifting logic Explanation: }The shifting logic is used to try out different positions for the yellow letters (the unknown letters that have been found but whose positions have not been identified yet) and see if any of them provide new information about the correct positions of the yellow letters. The function starts by finding all the yellow letters and their corresponding yellow positions. It then initializes a variable shift to zero and enters a loop that shifts the yellow positions by one position to the right in each iteration. The letters in currGuessFDict (which represent the guessed positions of the letters found so far) are updated according to the new shifted yellow positions. The shifting logic continues until new information is found or all possible shifts have been tried. The function then returns the updated wordleTracker object.

\textbf{Time Complexity:}
The time complexity of this algorithm is $O(k)$, where k is the length of the hidden word, assuming comparing guess word with hidden word is a constant time operation. This is because, in the worst case, we rotate by k times, placing each letter at all k positions once, and this gives us information about its correct location. We guess at max k words with each letter's position being shifted by 1 in each of those guess. So, time complexity is $O(k)$.

\textbf{Claim:} All anagrams are checked given k known letters, and the correct word is guessed.

\textbf{Proof:}
To prove the correctness of the algorithm, we can observe that it follows a simple strategy of finding all possible valid anagrams of the hidden word by iteratively guessing and checking letters in the correct positions.  Overall, this algorithm is guaranteed to find all possible anagrams of the hidden word by systematically trying out all possible combinations of letters and checking for correctness. Only anagrams are checked since the letter values are never changed. Thus, no extra words besides anagrams can be checked. The check of all possible anagrams is ensured by "shifting" the yellow letters in all possible positions until at least one of them turns green.

==> output.tex <==
\section{Output Formulation}
The game has two outputs. First output value is a Boolean which indicates if we were able to solve the game successfully. The second is an integer, which tells us the number of moves in which we solved the game. If we were unable to solve the game, the value of this is $-1$. Formally,\\
\begin{itemize}
    \item Boolean $is\_solved$ - $True$ if we solved the game in $l \le m$ moves i.e. $B[l].letters = h$, and $False$ otherwise.
   
    \item Integer $num\_moves$ - Denoting the number of chances $l$ we used to get to correct answer word $h$. $-1$ if we could not solve the game in $l \le m$ moves.
    
\end{itemize}

